Egocentric Video Task Translation

Different video understanding tasks are typically treated in isolation, and even with distinct types of curated data (e.g., classifying sports in one dataset, tracking animals in another). However, in wearable cameras, the immersive egocentric perspective of a person engaging with the world around them presents an interconnected web of video understanding tasks -- hand-object manipulations, navigation in the space, or human-human interactions -- that unfold continuously, driven by the person's goals. We argue that this calls for a much more unified approach. We propose EgoTask Translation (EgoT2), which takes a collection of models optimized on separate tasks and learns to translate their outputs for improved performance on any or all of them at once. Unlike traditional transfer or multi-task learning, EgoT2's flipped design entails separate task-specific backbones and a task translator shared across all tasks, which captures synergies between even heterogeneous tasks and mitigates task competition. Demonstrating our model on a wide array of video tasks from Ego4D, we show its advantages over existing transfer paradigms and achieve top-ranked results on four of the Ego4D 2022 benchmark challenges.

==> 4.exp_new.tex <==
\begin{table*}[!h]
  \centering
   % \resizebox{1.0\columnwidth}{!}{
\scalebox{0.8}{
  \begin{tabular}{l|cc|cc|cc}
    \toprule
& \multicolumn{2}{c}{$\mathcal T_p$ is LAM} & \multicolumn{2}{c}{$\mathcal T_p$ is TTM} & \multicolumn{2}{c}{$\mathcal T_p$ is ASD} \\
     & \makecell[c]{\# Params $\cdot 10^6$ \\ Trainable (\emph{All})} &  \makecell[c]{mAP\\ (\%)} & \makecell[c]{\# Params $\cdot 10^6$ \\ Trainable (\emph{All})} &  \makecell[c]{mAP\\ (\%)} & \makecell[c]{\# Params $\cdot 10^6$ \\ Trainable (\emph{All})} &  \makecell[c]{mAP \\ (\%)} \\
    \midrule
  TS model~\cite{ego4d} & 14.6 \emph{(14.6)} & 77.79 & 20.2  \emph{(20.2)} & 58.91 & 15.7 \emph{(15.7)} & 79.05\\
 \midrule 
 Fine-tuning~\cite{donahue2014decaf} & x & 78.14 & 0.8 \emph{(20.8)} & 59.67 & 1.1 \emph{(16.8)} & 78.62  \\
Transfer~\cite{zamir2018taskonomy} (LAM) & N/A & N/A & 0.8 \emph{(15.4)} & 63.59 & 1.6 \emph{(16.2)} & 66.40 \\
Transfer~\cite{zamir2018taskonomy} (TTM) & N/A & N/A & N/A & N/A & 1.6 \emph{(21.6)} & 71.06  \\
 Transfer~\cite{zamir2018taskonomy} (ASD) & N/A & N/A & 0.8 \emph{(16.5)} & 62.31 & N/A & N/A \\
 LF~\cite{ma2016going} (All Tasks) & N/A & N/A & 1.2 \emph{(51.5)} & 64.29 & 1.6 \emph{(51.9)} & 77.54\\
 \ett-s (All Tasks) & N/A & N/A & 0.7 \emph{(51.1)} & \textbf{66.54} & 1.5 \emph{(51.9)}& \textbf{79.38} \\
\hdashline
Multi-task~\cite{mtloverview} & 20.2 \emph{(20.2)} & 60.53 & 20.2 \emph{(20.2)} & 61.91 & N/A & N/A \\
 \ett-g (All Tasks) & 1.4 \emph{(51.7)} & 77.63 & 1.4 \emph{(51.7)} & 64.49 & 1.4 \emph{(51.7)} & 79.06 \\
 \bottomrule
  \end{tabular}
}
  \caption{Results of \ett-s for the primary task $\mathcal T_p$ being TTM and ASD, respectively. The first row records performance of the task-specific (TS) model we obtain in the first-stage training, and we compare \ett-s with other baseline methods in the second-stage training. `mAP' denotes mean Average Precision, and `LF' is short for Late Fusion. We list the number of trainable parameters for each separate stage as well as the total (\ie, trainable parameters plus parameters of frozen task-specific models) in parentheses.}
  \label{tab:hhi_new}
\end{table*}

\begin{table*}[!t]
  \centering
  \scalebox{0.75}{
 % \begin{small}{
  \begin{tabular}{lcc|cc|ccc|ccccc}
    \toprule
     & \multicolumn{2}{c}{$\mathcal T_p$ is PNR} & \multicolumn{2}{c}{$\mathcal T_p$ is OSCC} & \multicolumn{3}{c}{$\mathcal T_p$ is AR} & \multicolumn{5}{c}{$\mathcal T_p$ is LTA}   \\
     & \# Params $\cdot 10^6$ & Error & \# Params $\cdot 10^6$ & Acc. & \# Params $\cdot 10^6$ & \multicolumn{2}{c}{Acc. (\%)} & \# Params $\cdot 10^6$ & \multicolumn{2}{c}{Acc.(\%)}  & \multicolumn{2}{c}{ED@20} \\
     & Trainable (\emph{All}) & (s) & Trainable (\emph{All}) & (\%) & Trainable (\emph{All}) & Verb & Noun & Trainable (\emph{All}) & Verb & Noun  & Verb & Noun \\
    \midrule
  TS model ~\cite{ego4d} & 32.2 \emph{(32.2)} & 0.615 & 32.2 \emph{(32.2)} & 68.22 & 63.3 \emph{(63.3)} & \underline{22.18} & 21.55 & 180 \emph{(242)} & 20.82 & 21.80 & 0.746 & 0.789 \\
    \midrule
Fine-tuning~\cite{donahue2014decaf} & 8.4 \emph{(40.6)} & \underline{0.611} & 8.4 \emph{(40.6)} & 67.93 & 4.9 \emph{(66.8)} & 22.04 & 20.17 & 48.6 \emph{(266)} & 20.25 & 20.47 & \underline{0.744} & \underline{0.787} \\
    Transfer~\cite{zamir2018taskonomy} (PNR) & N/A & N/A & 8.4 \emph{(40.6)} & 66.80 & 4.9 \emph{(37.1)} & 20.09 & 5.35 & 65.4 \emph{(97.6)} & 20.81 & 10.97 & 0.778 & 0.902 \\
   Transfer~\cite{zamir2018taskonomy} (OSCC) & 8.4 \emph{(40.6)} & \underline{0.611} & N/A & N/A & 4.9 \emph{(37.1)} & 20.18 & 9.34 & 65.4 \emph{(97.6)} & 20.32 & 8.39 & 0.774 & 0.899  \\
 Transfer~\cite{zamir2018taskonomy} (AR) & 9.5 \emph{(71.4)} & 0.613 & 9.4 \emph{(71.4)} & 70.98 & N/A & N/A & N/A & 53.3 \emph{(115)} & \underline{21.26} & 21.48 & 0.753 & 0.798\\
 LF~\cite{ma2016going} (All Tasks) & 9.6 \emph{(135)} & \textbf{0.610} & 9.6 \emph{(135)} & \underline{72.10} & 5.2 \emph{(131)} & 21.79 & 18.54 & 83.6 \emph{(427)} &  20.76 & 21.08 & \underline{0.744} & 0.788 \\ %10.5 \emph{(136)} & 21.92 & 18.66
 \ett-s (All Tasks) & 6.4 \emph{(132)} & \textbf{0.610} & 7.4 \emph{(133)} & \textbf{72.69} & 4.3 \emph{(130)} & \textbf{23.04} & \underline{22.55} & 41.8 \emph{(348)} & 20.61 & \underline{22.36} &\textbf{0.731} & \textbf{0.769} \\  % 0.7269295893890222
 \hdashline
 Multi-task~\cite{mtloverview} & 32.2 \emph{(32.2)} & 0.617 & 32.2 \emph{(32.2)} & 66.01 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A\\
 \ett-g (PNR \& OSCC) & 5.9 \emph{(70.3)} & 0.612 & 5.9 \emph{(70.3)} & 68.58 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A  \\
 \ett-g (All Tasks) & 34.5 \emph{(378)} & \underline{0.611} & 34.5 \emph{(378)} & 71.65 & 34.5 \emph{(378)} & 21.93 & \bf{22.73} & 34.5 \emph{(378)} & \bf{21.91} & \bf{23.61} & N/A & N/A \\
    \bottomrule
  \end{tabular}
 }
 % \end{small}
  \caption{Results of \ett-s for the primary task $\mathcal T_p$ being PNR, OSCC, AR and LTA respectively. The evaluation metric is temporal localization error (unit: seconds) for PNR, accuracy for OSCC and AR and edit distance at future 20 time stamps (\ie, ED@20) for LTA. For localization error and ED@20, lower is better.}
  \label{tab:hoi_new}
\end{table*}


% `All Tasks' refers to LAM, TTM and ASD.
% \begin{table}[!h]
%   \centering
%   \resizebox{1.0\columnwidth}{!}{
%   \begin{tabular}{lcc}
%     \toprule
%     Method & \makecell[c]{\# Params\\ Trainable \emph{(All)}} &  \makecell[c]{mAP\\ (\%)} \\
%     \midrule
%  3D ResNet-18$^*$ & 20.2  \emph{(20.2)} & 58.91\\
%  \midrule 
%  fine-tuning & 0.8 \emph{(20.8)} & 59.67\\
%  Transfer (LAM) & 0.8 \emph{(15.4)} & 63.59 \\
%  Transfer (ASD) & 0.8 \emph{(16.5)} & 62.31 \\
%  Late Fusion (LAM + TTM + ASD) & 1.2 \emph{(51.5)} & 64.29\\
%  \ett \ (LAM + TTM + ASD) &0.7 \emph{(51.1)}& \textbf{66.54} \\
%  \bottomrule
%   \end{tabular}
%   }
%   \caption{Results on TTM. Auxiliary tasks are LAM and ASD. `mAP' denotes mean Average Precision. We list the number of trainable parameters (unit: million) required for each method for comparison and report all parameters involved (\ie, trainable parameters plus parameters of frozen task-specific models) as well.}
%   \label{tab:TTM}
% \end{table}

% \begin{table}[!h]
%   \centering
%   \resizebox{1.0\columnwidth}{!}{
%   \begin{tabular}{lcc}
%     \toprule
%     Method & \makecell[c]{\# Params\\ Trainable \emph{(All)}} &  \makecell[c]{mAP\\ (\%)} \\
%     \midrule
% TalkNet$^*$ & 15.7 \emph{(15.7)} & 79.05 \\
%  \midrule 
%  fine-tuning & 1.1 \emph{(16.8)} & 78.62\\
%  Transfer (LAM) & 1.6 \emph{(16.2)} & x \\ %70.49 \\
%  Transfer (TTM) & 1.6 \emph{(21.6)} & x \\ %76.22 \\
%  Late Fusion (LAM + TTM + ASD) & 1.6 \emph{(51.9)} & 77.13 \\
% %   \ett \ (TTM + ASD) & 1.4 \emph{(51.8)} & 78.89 \\
%  \ett \ (LAM + TTM + ASD) & 1.5 \emph{(51.9)}& \textbf{79.38} \\
%  \bottomrule
%   \end{tabular}
%   }
%   \caption{Results on ASD. Auxiliary tasks are LAM and TTM.}
%   \label{tab:ASD}
% \end{table}

% \begin{table}[!h]
%   \centering
%   \resizebox{1.0\columnwidth}{!}{
%   \begin{tabular}{lcc}
%     \toprule
%     Method & \makecell[c]{\# Params\\ Trainable \emph{(All)}} &  \makecell[c]{Loc.\\ Err. (s)} \\
%     \midrule
%     I3D ResNet-50$^*$ & 32.2 \emph{(32.2)} & 0.615 \\
%     SViT~\cite{ben2022structured}  & x &  0.640\\
%     Video Swin Transformer~\cite{liu2022video} & x & 0.61\\
%     Frozen~\cite{bain2021frozen} with V-T pretraining & x & 0.611\\
%     \midrule
%     fine-tuning & 8.4 \emph{(40.6)} & 0.611\\
%     Transfer (OSCC) & 8.4 \emph{(40.6)} & 0.611\\
%     Transfer (AR) & 9.5 \emph{(71.4)} & 0.613\\
%     Late Fusion (PNR + OSCC + AR) & 9.6 \emph{(135)} & 0.610 \\
%     \hdashline
%     \ett \ (PNR + OSCC) & 5.8 \emph{(70.2)} & \textbf{0.610} \\ %0.6077
%     \ett \ (PNR + OSCC + AR) & 6.4 \emph{(132)} & 0.610\\  %0.6104
%     \bottomrule
%   \end{tabular}}
%   \caption{Results on PNR. OSCC and AR are adopted as auxiliary tasks. The evaluation metric is localization error (seconds). The upper table lists state-of-the-art methods to obtain a PNR model, where the one with a $*$ (\ie, I3D ResNet-50) denotes our choice of the task-specific model in \ett. The lower table compares different approaches to utilize pretrained models to further improve the PNR task. }
%   \label{tab:PNR}
% \end{table}

% \begin{table}[!h]
%   \centering
%   \resizebox{1.0\columnwidth}{!}{
%   \begin{tabular}{lcc}
%     \toprule
%     Method & \makecell[c]{\# Params\\ Trainable \emph{(All)}} &  \makecell[c]{Acc.\\ (\%)} \\
%     \midrule
%     I3D ResNet-50$^*$ & 32.2 \emph{(32.2)} & 68.2 \\
%     Video Swin Transformer~\cite{liu2022video} & x & 69.5\\
%     Deformable Swin~\cite{escobar2022video} & x & 69.8\\
%     TimeSformer ~\cite{islam2022object} & x & 70.8\\
%     Frozen~\cite{bain2021frozen} with V-T pretraining & 172.2 \emph{(172.2)} & 73.9\\
%     \midrule
%     fine-tuning & 8.4 \emph{(40.6)} & 67.9\\
%     Transfer (PNR) & 8.4 \emph{(40.6)} & 66.8\\
%     Transfer (AR) & 9.4 \emph{(71.4)} & 71.0\\
%     Late Fusion (PNR + OSCC + AR)  & 9.6 \emph{(135)} & 72.1 \\
%     \hdashline
%     \ett \ (PNR + OSCC + AR) & 7.4 \emph{(133)} & \textbf{72.5}\\ 
%     \bottomrule
%   \end{tabular}}
%   \caption{Results on OSCC. PNR and AR are auxiliary tasks.  \KG{here and above, split out the in-house comparisons from the SoTA comparisons?}}
%   \label{tab:OSCC}
% \end{table}

% \begin{table*}[!t]
%   \centering
%   \begin{small}{
% %   \resizebox{1.4\columnwidth}{!}{
%   \begin{tabular}{lccc}
%     \toprule
%     Method & \makecell[c]{\# Params\\ Trainable \emph{(All)}} & \makecell{Verb\\ Acc. (\%)} & \makecell{Noun\\ Acc. (\%)} \\
%     \midrule
%     SlowFast$^*$ & 63.3 \emph{(63.3)} & 22.06 & 20.95 \\
%     \midrule
%     fine-tuning & 4.9 \emph{(66.8)} & 22.04 & 20.17 \\
%     Transfer (PNR) & 4.9 \emph{(37.1)} & 20.09 & 5.35\\
%     Transfer (OSCC) & 4.9 \emph{(37.1)} & 20.18 & 9.34 \\
%     Transfer (LTA$^\dag$) & 4.8 \emph{(222)} & 21.66 & 22.77 \\
%     Late Fusion (PNR + OSCC + AR) & 5.2 \emph{(131)} & 21.79 & 18.54\\
%     \hdashline
%     \ett \ (AR + LTA$^\dag$) & 2.4 \emph{(282)} & 22.24 & \textbf{23.11} \\
%     \ett \ (PNR + OSCC + AR) & 4.3 \emph{(130)} & \textbf{23.04} & 22.55 \\
%     \bottomrule
%   \end{tabular}
%   }\end{small}
% %   }
%   \caption{Results on AR. Auxiliary tasks are PNR and OSCC. Additionally, we expand the input video of AR datasets from 8 seconds to 16 seconds to make the task-specific LTA model (that work on 16-seconds long video) applicable. The results obtained with expanded video length and LTA features are marked with $^\dag$.}
%   \label{tab:AR}
% \end{table*}

% \begin{table*}[!t]
%   \centering
%   \begin{small}{
% %   \resizebox{1.4\columnwidth}{!}{
%   \begin{tabular}{lccc}
%     \toprule
%     Method & \makecell[c]{\# Params\\ Trainable \emph{(All)}} & \makecell{Verb\\ ED@20} & \makecell{Noun\\ ED@20} \\
%     \midrule
%     SlowFast$^*$ & 180 \emph{(242)} & 0.746 & 0.789 \\
%     \midrule
%     fine-tuning & 48.6 \emph{(266)} & 0.744 & 0.787\\
%     Transfer (PNR) & 65.4 \emph{(97.6)} & 0.778 & 0.902 \\
%     Transfer (OSCC) & 65.4 \emph{(97.6)} & 0.774 & 0.899 \\
%     Transfer (AR) & 53.3 \emph{(115)} & 0.745 & 0.806 \\
%     Late Fusion (PNR + OSCC + AR + LTA) & 83.6 \emph{(427)} & 0.744 & 0.788 \\
%     \hdashline
%     \ett \ (AR + LTA) & 54.2 \emph{(296)} & \textbf{0.727} & 0.778 \\
%     \ett \ (PNR + OSCC + AR + LTA) & 41.8 \emph{(348)} & 0.731 & \textbf{0.769} \\
%     \bottomrule
%   \end{tabular}
%   }\end{small}
% %   }
%   \caption{Results on LTA. Auxiliary tasks are PNR, OSCC and AR. The evaluation metric is edit distance at future 20 time stamps (\ie, ED@20); lower is better.}
%   \label{tab:LTA}   
% \end{table*}

% \begin{table*}[!t]
%   \centering
%    \begin{small}{
%   \begin{tabular}{llccc|ccc}
%     \toprule
%     & & \multicolumn{3}{c}{$\mathcal T_p$ is AR} & \multicolumn{3}{c}{$\mathcal T_p$ is LTA} \\
%     & & \makecell[c]{\# Params $\cdot 10^6$} & \makecell[c]{V. Acc. (\%)} & \makecell[c]{N. Acc. (\%)} & \# Params $\cdot 10^6$ & \makecell[c]{V. ED@20} & \makecell[c]{N. ED@20} \\
%     \midrule
% Stage I & Task-specific model~\cite{ego4d} & 63.3 \emph{(63.3)} & 22.06{\color{white}$^\star$} & 20.95{\color{white}$^\star$} & 180 \emph{(242)} & 0.746 & 0.789 \\
%     \midrule
%   \multirow{8}{*}{Stage II} & Fine-tuning~\cite{donahue2014decaf} & 4.9 \emph{(66.8)} & 22.04{\color{white}$^\star$} & 20.17{\color{white}$^\star$} & 48.6 \emph{(266)} & 0.744 & 0.787\\
%     & Transfer~\cite{zamir2018taskonomy} (PNR) & 4.9 \emph{(37.1)} & 20.09{\color{white}$^\star$} & 5.35{\color{white}$^\star$} & 65.4 \emph{(97.6)} & 0.778 & 0.902 \\
%     & Transfer~\cite{zamir2018taskonomy} (OSCC) & 4.9 \emph{(37.1)} & 20.18{\color{white}$^\star$} & 9.34{\color{white}$^\star$} & 65.4 \emph{(97.6)} & 0.774 & 0.899  \\
%     & Transfer~\cite{zamir2018taskonomy} (AR) & N/A & N/A{\color{white}$^\star$} & N/A{\color{white}$^\star$} & 53.3 \emph{(115)} & 0.745 & 0.806 \\
%     & Transfer~\cite{zamir2018taskonomy} (LTA) & 4.8 \emph{(222)} & 21.66$^\star$ & 22.77$^\star$ & N/A & N/A & N/A \\
%     % & Late Fusion~\cite{ma2016going} (PNR + OSCC + AR) & 5.2 \emph{(131)} & 21.79 & 18.54 & - & - & - \\
%     % & Late Fusion~\cite{ma2016going} (PNR + OSCC + AR + LTA) & - & - & - & 83.6 \emph{(427)} & 0.744 & 0.788 \\
%     & Late Fusion~\cite{ma2016going} (All Tasks) & 5.2 \emph{(131)} & 21.79{\color{white}$^\star$} & 18.54{\color{white}$^\star$} & 83.6 \emph{(427)} & 0.744 & 0.788 \\
%     & \ett-s (AR + LTA) & 2.4 \emph{(282)} & 22.24$^\star$ & \textbf{23.11}$^\star$ & 54.2 \emph{(296)} & \textbf{0.727} & 0.778 \\
%     & \ett-s (All Tasks) & 4.3 \emph{(130)} & \textbf{23.04}{\color{white}$^\star$} & 22.55{\color{white}$^\star$} & 41.8 \emph{(348)} & 0.731 & \textbf{0.769} \\
%     \bottomrule
%   \end{tabular}
%   }\end{small}
%   \caption{Results of \ett-s for the primary task $\mathcal T_p$ being AR and LTA, respectively. `V' and `N' represent verb and noun, respectively. The evaluation metric for LTA is verb and noun edit distance at future 20 time stamps (\ie, ED@20); lower is better. The results achieved with expanded input video length are marked with a $^\star$. `All Tasks' refer to PNR, OSCC and AR if $\mathcal T_p$ is AR and PNR, OSCC, AR and LTA if $\mathcal T_p$ is LTA.}
%   \label{tab:ts_HOI2}
% \end{table*}

% We conduct experiments of \ett-s for each human-object interaction task being the primary task and summarize results in Table \ref{tab:ts_HOI1}-\ref{tab:ts_HOI2}. As shown in Table \ref{tab:dataset}, the LTA task-specific backbone requires videos of 16 seconds while the other three tasks operate on videos of 8 seconds. Therefore, when primary task is LTA, we slide the other task-specific backbones along the 16-seconds time window to obtain auxiliary task features; the stride size is set to 8 seconds. When the primary task is PNR, OSCC or AR, LTA is not a valid auxiliary task since its task-specific model requires video of a longer temporal span than provided in these three datasets. In fact, it is possible to expand the input video length of the AR dataset to be 16 seconds. To thoroughly evaluate \ett, we also conduct experiments with this setup and mark results obtained by using longer input video with a $^\star$ in Table \ref{tab:ts_HOI2}.

% \begin{table*}[!t]
%   \centering
%  \begin{small}{
%   \begin{tabular}{llcc|cc}
%     \toprule
%     &  & \multicolumn{2}{c}{$\mathcal T_p$ is PNR} & \multicolumn{2}{c}{$\mathcal T_p$ is OSCC} \\
%     & & \makecell[c]{\# Params $\cdot 10^6$} & \makecell[c]{Err. (s)} & \makecell[c]{\# Params $\cdot 10^6$} & \makecell[c]{Acc. (\%)}\\
%     \midrule
%    Stage I & Task-specific model ~\cite{ego4d} & 32.2 \emph{(32.2)} & 0.615 & 32.2 \emph{(32.2)} & 68.2 \\
%     \midrule
%   \multirow{6}{*}{Stage II} & Fine-tuning~\cite{donahue2014decaf} & 8.4 \emph{(40.6)} & 0.611 & 8.4 \emph{(40.6)} & 67.9 \\
%    & Transfer~\cite{zamir2018taskonomy} (PNR) & N/A & N/A & 8.4 \emph{(40.6)} & 66.8\\
%    & Transfer~\cite{zamir2018taskonomy} (OSCC) & 8.4 \emph{(40.6)} & 0.611 & N/A & N/A\\
%    & Transfer~\cite{zamir2018taskonomy} (AR) & 9.5 \emph{(71.4)} & 0.613 & 9.4 \emph{(71.4)} & 71.0\\
%    & Late Fusion~\cite{ma2016going} (All Tasks) & 9.6 \emph{(135)} & 0.610 & 9.6 \emph{(135)} & 72.1\\
%    & \ett-s \ (All Tasks) & 6.4 \emph{(132)} & \textbf{0.610} & 7.4 \emph{(133)} & \textbf{72.7}\\  % 0.7269295893890222
%     \bottomrule
%   \end{tabular}
%  }\end{small}
%   \caption{Results of \ett-s \ for the primary task $\mathcal T_p$ being PNR and OSCC, respectively. The evaluation metric is temporal localization error (seconds) for PNR and accuracy for OSCC. `All Tasks' denotes PNR, OSCC and AR.}
%   \label{tab:ts_HOI1}
% \end{table*}

% \begin{table*}[!t]
%   \centering
%    \begin{small}{
%   \begin{tabular}{llccc|ccc}
%     \toprule
%     & & \multicolumn{3}{c}{$\mathcal T_p$ is AR} & \multicolumn{3}{c}{$\mathcal T_p$ is LTA} \\
%     & & \makecell[c]{\# Params $\cdot 10^6$} & \makecell[c]{V. Acc. (\%)} & \makecell[c]{N. Acc. (\%)} & \# Params $\cdot 10^6$ & \makecell[c]{V. ED@20} & \makecell[c]{N. ED@20} \\
%     \midrule
% Stage I & Task-specific model~\cite{ego4d} & 63.3 \emph{(63.3)} & 22.06{\color{white}$^\star$} & 20.95{\color{white}$^\star$} & 180 \emph{(242)} & 0.746 & 0.789 \\
%     \midrule
%   \multirow{8}{*}{Stage II} & Fine-tuning~\cite{donahue2014decaf} & 4.9 \emph{(66.8)} & 22.04{\color{white}$^\star$} & 20.17{\color{white}$^\star$} & 48.6 \emph{(266)} & 0.744 & 0.787\\
%     & Transfer~\cite{zamir2018taskonomy} (PNR) & 4.9 \emph{(37.1)} & 20.09{\color{white}$^\star$} & 5.35{\color{white}$^\star$} & 65.4 \emph{(97.6)} & 0.778 & 0.902 \\
%     & Transfer~\cite{zamir2018taskonomy} (OSCC) & 4.9 \emph{(37.1)} & 20.18{\color{white}$^\star$} & 9.34{\color{white}$^\star$} & 65.4 \emph{(97.6)} & 0.774 & 0.899  \\
%     & Transfer~\cite{zamir2018taskonomy} (AR) & N/A & N/A{\color{white}$^\star$} & N/A{\color{white}$^\star$} & 53.3 \emph{(115)} & 0.745 & 0.806 \\
%     & Transfer~\cite{zamir2018taskonomy} (LTA) & 4.8 \emph{(222)} & 21.66$^\star$ & 22.77$^\star$ & N/A & N/A & N/A \\
%     % & Late Fusion~\cite{ma2016going} (PNR + OSCC + AR) & 5.2 \emph{(131)} & 21.79 & 18.54 & - & - & - \\
%     % & Late Fusion~\cite{ma2016going} (PNR + OSCC + AR + LTA) & - & - & - & 83.6 \emph{(427)} & 0.744 & 0.788 \\
%     & Late Fusion~\cite{ma2016going} (All Tasks) & 5.2 \emph{(131)} & 21.79{\color{white}$^\star$} & 18.54{\color{white}$^\star$} & 83.6 \emph{(427)} & 0.744 & 0.788 \\
%     & \ett-s \ (AR + LTA) & 2.4 \emph{(282)} & 22.24$^\star$ & \textbf{23.11}$^\star$ & 54.2 \emph{(296)} & \textbf{0.727} & 0.778 \\
%     & \ett-s \ (All Tasks) & 4.3 \emph{(130)} & \textbf{23.04}{\color{white}$^\star$} & 22.55{\color{white}$^\star$} & 41.8 \emph{(348)} & 0.731 & \textbf{0.769} \\
%     \bottomrule
%   \end{tabular}
%   }\end{small}
%   \caption{Results of \ett-s \ for the primary task $\mathcal T_p$ being AR and LTA, respectively. `V' and `N' represent verb and noun, respectively. The evaluation metric for LTA is verb and noun edit distance at future 20 time stamps (\ie, ED@20); lower is better. The results achieved with expanded input video length are marked with a $^\star$. `All Tasks' refer to PNR, OSCC and AR if $\mathcal T_p$ is AR and PNR, OSCC, AR and LTA if $\mathcal T_p$ is LTA.}
%   \label{tab:ts_HOI2}
% \end{table*}

% \begin{table}[!h]
%   \centering
%   \scalebox{0.8}{
% % \resizebox{1.0\columnwidth}{!}{
%   \begin{tabular}{lc|ccc}
%     \toprule
%     & Params $\cdot 10^6$ & LAM & TTM & ASD \\
%     \midrule
%     TS model (LAM)~\cite{ego4d} & 14.6 \emph{(14.6)} & \textbf{77.79} & N/A & N/A \\
%     TS model (TTM)~\cite{ego4d} & 20.2 \emph{(20.2)} & N/A & 58.91 & N/A \\
%     TS model (ASD)~\cite{ego4d} & 15.7 \emph{(15.7)} & N/A & N/A & \underline{79.05}\\
%     \midrule
%    Hard parameter sharing~\cite{mtloverview} & 20.2 \emph{(20.2)} & 60.53 & \underline{61.91} &  N/A \\
%     % \ett \ (LAM \& TTM) & x & & &\\
%     \ett-g (All Tasks) & 1.4 \emph{(51.7)} & \underline{77.63} & \textbf{64.49} & \textbf{79.06}\\
%     \bottomrule
%   \end{tabular}
% }
%   \caption{\ett-g for human-human interaction tasks. The evaluation metric is mAP (\%) for LAM and TTM and accuracy (\%) for ASD. The best results are bolded are the second best results are underlined. Hard parameter sharing is implemented by sharing a backbone (\ie, 3D ResNet-18) and having two separate prediction heads for LAM and TTM.}
%   \label{tab:HHI}
% \end{table}

% \begin{table*}[!h]
%   \centering
% \scalebox{0.8}{
%   \begin{tabular}{lc|cccccc}
%     \toprule
%     & Params $\cdot 10^6$ & PNR & OSCC & AR Verb & AR Noun & LTA Verb & LTA Noun \\
%     \midrule
%    TS model (PNR)~\cite{ego4d} & 32.2 \emph{(32.2)} & 0.615 & N/A & N/A & N/A & N/A & N/A \\
%    TS model (OSCC)~\cite{ego4d} & 32.2 \emph{(32.2)} & N/A & 68.2 & N/A & N/A & N/A & N/A \\
%    TS model (AR)~\cite{ego4d} & 63.3 \emph{(63.3)} & N/A & N/A & \textbf{22.06} & \underline{20.95} & N/A & N/A \\
%    TS model (LTA)~\cite{ego4d} & 180 \emph{(242)} & N/A & N/A & N/A & N/A & \textbf{21.26} & \underline{21.75} \\ % \emph{(218)}
%   \midrule 
%    Hard parameter sharing~\cite{mtloverview} & 32.2 \emph{(32.2)} & 0.617 & 66.0 & N/A & N/A & N/A & N/A \\
%      \ett-g (PNR \& OSCC) & 5.9 \emph{(70.3)} & \underline{0.612} & \underline{68.58} & N/A & N/A & N/A & N/A\\
%    \ett-g (All Tasks) & 34.5 \emph{(378)} & \textbf{0.611} & \textbf{71.7} & \underline{21.81} & \textbf{22.38} & \underline{20.83} & \textbf{22.38}\\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{\ett-g for human-object interaction tasks. We report localization error (seconds) for PNR and accuracy (\%) for the other tasks. Hard parameter sharing is implemented by sharing a backbone (\ie, SlowFast) and having two separate prediction heads for PNR and OSCC. \LT{Perhaps use `Multi-task' to denote the baseline (the explanation of shared backbone and separate heads is in the text.}\SX{Will multi-task seem too general? Shall we use hard parameter sharing?} \LT{As long as we explain it in the text it's fine. Here it's more important to clarify the approach of the baseline rather than the specific design.}\LT{There are a lot of N/A in this table. I think it stems from havint to list different number of parameters for each model. How about omitting altogether the number of parameters from this table and organize TS results in a single row? We can state that the number of parameters for each model is listed in the supplementary. Same for Table 6.}}
%   \label{tab:HOI}
% \end{table*}
